When Interactive Graphic Storytelling Fails

Many people are unaware of the digital dangers that lie around each cyber-corner. Teaching people how to recognize dangerous situations is crucial, especially for those who work on or with computers. We postulated that interactive graphic vignettes could be a great way to expose professionals to dangerous situations and demonstrate the effects of their choices in these situations. In that way, we aimed to inoculate employees against cybersecurity threats. We used the Comic-BEE platform to create interactive security awareness vignettes and evaluated for how employees of a major industrial company perceived them. For analysing the potential of these comics, we ran an evaluation study as part of a capture-the-flag (CTF) event, an interactive exercise for hacking vulnerable software. We evaluated whether the comics fulfilled our requirements based on the responses of the participants. We showed the comics, on various cybersecurity concepts, to 20 volunteers. In the context of a CTF event, our requirements were not fulfilled. Most participants considered the images distracting, stating a preference for text-only material.

==> 2-background.tex <==
\section{Background}


%What is the best method for teaching?
Learning theories have come a long way since Socrates; but most of the empirically valid work has been done after 1960 \cite{Glaser1965TeachingII}.
This paper is concerned with how to design instructional material, and how it can be applied to the company and other institutions like it.
Wilson \& Cole (\citeyear{Wilson1996CognitiveModels}) wrote a chapter on the progress of Instructional Design, as understood through the lens of cognitive models: from the 1960's, with Behavioral psychology; through Information Processing psychology in the 1970's and 1980's; to the 1990's and the present, which emphasizes the construction of knowledge and the role of social mediation.
The state of the art is now considered to be "Constructivism," which has been the predominant learning theory over the past three decades \cite{Fosnot1996CONSTRUCTIVISM:Learning}.
Constructivism presupposes two main tenets: (1) knowledge is a construction that comes from an active interaction with the world, and (2) that it is inherently an adaptive process that is not necessarily concerned with the ontological nature of reality.

Building on these facts, we next consider the visceral experience of the learner.
Sweller (\citeyear{Sweller1994CognitiveDesign}) considered the factors that make learning more or less difficult; especially, when you have two subjects with similar amounts of information, but one requires much more effort to understand, while the other seems to be readily absorbed.
He found that subject matter can be presented in such a way that the information enters several channels and thus diminishes the amount of strain, or load, put on "cognition."
% \blockquote{``There are two critical learning mechanisms: schema acquisition and the transfer of learned procedures from controlled to automatic processing. It will be argued that intellectual mastery of any subject matter is overwhelmingly dependent on these two processes'' 
% \cite[p. 296]{Sweller1994CognitiveDesign}}
This paper attempts to address human learning at the psychological level, therefore it looks at the substrates of learning, i.e., the media (and multimedia) that is passing information to the learner.

This paper combines the multimedia theory of learning and a Constructivist approach so that learners will be shown information that they can readily comprehend, then engage with to form even stronger memories about what to do in various cybersecurity situations.
Additionally, they will form conceptions about the consequences of their decisions, something that is missing from many training sessions, and is found to be missing in education generally.

This paper is concerned with how to design instructional material, which falls under the subset of learning theories that are about instructional design; and how it can be applied to the company and other institutions like it.
Wilson \& Cole \citeyear{Wilson1996CognitiveModels} wrote about the progress of Instructional Design over the past few decades, from the perspective of cognitive models: the 1960's saw the rise of Behavioral psychology; then came Information Processing psychology in the 1970's and 1980's; to the 1990's and the present, which emphasizes the construction of knowledge and social mediation.
The state of the art is now considered to be "Constructivism," which has been the predominant learning theory over the past three decades \cite{Fosnot1996CONSTRUCTIVISM:Learning}.
Constructivism presupposes two main tenets: (1) knowledge is a construction that comes from an active interaction with the world, and (2) that it is inherently an adaptive process that is not necessarily concerned with the ontological nature of reality. We address these tenets by (1) having our participants make active choices in the stories they interact with and (2) utilizing fictional stories that express larger truths about cybersecurity.

The authors then consider the visceral experience of the learner.
Sweller (\citeyear{Sweller1994CognitiveDesign}) investigated the factors that make learning more or less difficult; especially, when there are two subjects with similar amounts of information, but one requires much more effort to understand, while the other seems to be readily absorbed.
He found that subject matter can be presented in such a way that the information enters several channels and thus diminishes the amount of strain, or load, put on "cognition."
% \blockquote{``There are two critical learning mechanisms: schema acquisition and the transfer of learned procedures from controlled to automatic processing. It will be argued that intellectual mastery of any subject matter is overwhelmingly dependent on these two processes'' 
% \cite[p. 296]{Sweller1994CognitiveDesign}}
This paper attempts to address human learning at this psychological level by looking at the substrates of learning, i.e., the media (and multimedia) that is passing information to the learner.

This paper combines the Multimedia Theory of learning and a Constructivist approach so that learners will be shown information that they can readily comprehend, then engage with to form even stronger memories about what to do in various cybersecurity situations.
Additionally, they will form conceptions about the consequences of their decisions, something that is missing from many training sessions, and is found to be missing in education generally.

%\subsection{Constructivism}

%\subsection{Cognitive Load}

%\subsection{Situated Learning}

%\subsection{Alternative forms Education} i.e., CTFs and comics

\section{Related Work}

Comics have been used before to teach about complex issues, such as training soldiers on matters of military leadership \cite{gordon2006}. These comics consisted of four panels, the first three setting up a problem to be solved or a situation that may be encountered in the field. The last panel then was empty, and participants would fill in a response. Finally, there was a forum that included previous responses so that these could be discussed. Our work does not utilize forums, and the interaction is multiple choice, as opposed to a short answer response. This allows for more immediate feedback and for a variety of outcomes to be explored.

Security training has often been perceived as  uninteresting and even boring. Therefore, several researchers have been developing serious games to combine entertainment and training in this field. 
\textit{CyberCIEGE}~\cite{irvine2005cyberciege} is a role playing video game, where players act as an information security decision maker of a company. Players have to minimize risk, while continuing to work. \textit{PlayingSafe} ~\cite{newbould2009playing} consists of multiple choice questions about cybersecurity, using the typical mechanics of a board game. \textit{SEAG}~\cite{olanrewajusocial} is also using multiple choice questions and in addition players have to match cybersecurity terms with respective pictures. Our work differs since none of these approaches use comic-based vignettes based on real industry concerns.

And in terms of generating comics, Microsoft has done some very interesting work on automatically generated comics based on cursory language analysis \cite{Kurlander1996}. Their goals were not to produce training material, but to visually represent chat environments to enrich the user experience and make electronic chat rooms more dynamic and interesting. While this technology may be incorporated into future renditions of our work, all of our comics were generated "by hand."

The case for using such a platform as Comic-BEE to create comics is laid out in \cite{Ledbetter2016CySComYouth}. The stated goals and objectives therein was to introduce young people to cybersecurity content in a fun and engaging way, in an effort to encourage them to pursue cybersecurity career paths. Among the reasons they cite are that (1) educational comics can be appealing on multiple levels, including engaging and increasing interest in readers; and (2) young people are not being sufficiently exposed to  cybersecurity concepts, even while they are ever more surrounded by technology. What we would like to do is take these concepts into an industrial workplace to test whether the claims of interest and engagement hold up for a more mature audience. 




==> Settings/conf.tex <==
\captionsetup[table]{justification=raggedright,singlelinecheck=off}
\sisetup{separate-uncertainty=true}

%\addto\extrasenglish{%
%  \renewcommand{\subsectionautorefname}{section}%
%}

%\addto\extrasenglish{%
%  \renewcommand{\subsubsectionautorefname}{section}%
%}

\newcolumntype{P}[1]{>{\RaggedRight\hspace{0pt}}p{#1}}

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

% Path for graphics
\graphicspath{{figures/}}
